Graph-based Ontology Summarization: A Survey

Ontologies have been widely used in numerous and varied applications, e.g., to support data modeling, information integration, and knowledge management. With the increasing size of ontologies, ontology understanding, which is playing an important role in different tasks, is becoming more difficult. Consequently, ontology summarization, as a way to distill key information from an ontology and generate an abridged version to facilitate a better understanding, is getting growing attention. In this survey paper, we review existing ontology summarization techniques and focus mainly on graph-based methods, which represent an ontology as a graph and apply centrality-based and other measures to identify the most important elements of an ontology as its summary. After analyzing their strengths and weaknesses, we highlight a few potential directions for future research.

==> 2Preliminaries.tex <==
%\section{Ontology Summarization}
%As the size and the complexity of ontologies increase, there is a high demand in order to facilitate ontology understanding and help users take advantage of an ontology quickly. There are ontology management \cite{hepp2007ontology} techniques that aim to reduce the size and complexity of an ontology such as ontology partitioning \cite{d2007ontology}, ontology segmentation \cite{seidenberg2006web}  , and ontology modularization \cite{stuckenschmidt2009modular} but, they do not keep the most important information. Differently, ontology summarization attempt to provide efficient and effective models to grab knowledge from an ontology while preserving informative nodes. The expected outcome of ontology summarization, usually, is defined as sub-graphs or key nodes at the data and schema level that represents the most important nodes (entities or concepts). 

% Ontology is a key point in the deployment and development of the Semantic Web. Ontologies enable organizing and information sharing on the Web by the capability of specifying a shared conceptualization explicitly\cite{gruber1993translation}. In fact, an ontology provides a basic structure of knowledge for a specific domain \cite{queiroz2013method} that can be reused in order to develop a new ontology, they are increasingly difficult to be understood. One effective approach that enables a better ontology understanding is the process of ontology summarization. Usually, the ultimate goal of ontology summarization technique is providing an abridged ontology that contains the most relevant concept within an ontology.
%****************************************************************************************

==> 5Approaches.tex <==
\section{Ontology Summarization Techniques }
\textcolor{red}{I am not sure whether we need this section, or how we should structure this section. I will think about it tomorrow.}

Ontology summarization is usually considered as an effective way to understand an ontology in order to support different tasks such as ontology reusing in ontology construction development. In literatures, ontology summarization is referred to extractive summarization approach in which the important concepts (at the schema layer) and important entities (at the data layer) are extracted and represented as a summary of an ontology. Based on different measurements in the section \ref{assess}, various methods in ontology summarization have been proposed which are highlighting different criterias to generate a summary for an ontology. In the next section, we are primarily focusing on the approaches which are dedicated in \emph{Ontology Summarization} and providing more details about them. Additionally, Table \ref{OntoSum} represents an overview of the models, the measures and the expected outcome for each model.



\iffalse
%\begin{landscape}
\begin{table*}[!th]
	% \centering
	% \setlength{\floatsep}{1.25\baselineskip plus 3pt minus 2pt}
	% \captionsetup{justification=centering} 
	\caption{Ontology Summarization Models, Measures, and expected outcomes.}
	\resizebox{\linewidth}{!}{% 
		\begin{threeparttable}
			\begin{tabular}{l cccccccccccccccc ll}
				\toprule
				& \multicolumn{16}{c}{\textbf{Measures}} &  \\
				\cmidrule(lr){2-17} 
				\textbf{Model}     &  DC\tnote{1}      &
				CC\tnote{2}   & 
				BC\tnote{3}   & 
				BrC\tnote{4}    & 
				HC\tnote{5}   & 
				Ra\tnote{6}   &
				EgC\tnote{7}   & 
				RC\tnote{8}   &
				Re\tnote{9}   &
				EC\tnote{10}   &
				Fr\tnote{11}   &
				NS\tnote{12}   &
				De\tnote{13}    &
				Co\tnote{14}    &
				Po\tnote{15}    & 
				Ref\tnote{16}    &
				
				\textbf{Outcome}&\textbf{Note}  \\
				\midrule
				\cite{pappas2017exploring}  & \cmark{}  & -  & \cmark{}     & \cmark{}  & \cmark{}   &\cmark{}  &  \cmark{}   & - & - & - &  -  &  - & -   & -  &-    &- & sub-schema graph      & Normalize each importance measure and use \emph{adopted importance measure} \\
				\hline
				\cite{queiroz2013method}  & \cmark{} & \cmark{} & - & - & - &-  &  -  & -     & \cmark{}     & - &   -  &  -&-   & - & -&-   &Sub-schema graph      &Ontology summary size is defined by a user \\
				\hline
				
				\cite{zhang2007ontology,zhang2009summarizing}    &\cmark{} & -  & \cmark{}     & -{}  & -{}   &-& -  & -    & -     & \cmark{} &  -  &  -&-   & -            & - &-  &RDF graph       & The weighted version of \emph{PageRank} and \emph{HITS} algorithem were applied.             \\
				\hline
				
				\cite{troullinou2017ontology}     & \cmark{}     & -  & -     & -  & -   &-              &  -   & \cmark{}     & \cmark{}     & -  &   -   &  - &-    & -             & -  &-   &Sub-schema graph      &             \\
				\hline
				
				\cite{pires2010summarizing}     & \cmark      & -  & -     & -  & -   &-              &  -   & -      & \cmark      & -  &  \cmark   &  - &-    & -  & - &-    &Sub-schema graph      &              \\
				\hline
				
				\cite{peroni2008identifying}     & -      & -  & -     & -  & -   &- &  -   & - & - &-  &   -   &  \cmark &\cmark    & \cmark& -  &-   &Sub-graph      &             \\
				\hline
				\cite{li2010ontology}     & -     &  - &  -    &  - &  -  & -  &   -  &  -     &  -     &  -  &    -  & -{}&\cmark{}   & \cmark{}  & \cmark{} &\cmark{}  &Key concepts      &
				
				Using \emph{structural}  and \emph{linguistic} features of ontology \\
				\hline
				
				\cite{troullinou2015rdf}     & \cmark     & -             & -    & - & -  &-             &  -  & \cmark     & \cmark     & -             &   -  &  -&-   & \cmark            & - &-  &RDF graph      &-              \\
				\hline
				
				%     \cite{hlomani2014approaches}     & b     & c             & d    & e & f  &g             &  h  & i     & j     & k             &   l  &  m&n   & o            & p &0  &q      &r              \\
				%     \hline
				
				\cite{zhang2011degree}     & \cmark     & -             & -    & - & -  &-             &  -  & -     & -     & -             &   -  &  -&-   & -            & - &-  &RDF graph      &-              \\
				
				\hline 
				\cite{ereteo2009semantic}     & \cmark     & \cmark             & \cmark    & - & -  &-             &  -  & -     & -     & -             &   -  &  -&-   & -            & - &-  &Sub-graph      &-              \\
				
				\hline
				\cite{hsi2003ontological}     & \cmark     & \cmark            & \cmark   & - & -  &-             &  -  & -     & -     & \cmark             &   -  &  -&-   & -            & - &-  &Core concepts      &-              \\
				
				\hline
				\cite{ereteo2008state}     & \cmark     & \cmark            & \cmark   & - & -  &-             &  -  & -     & -     & -             &   -  &  -&\cmark   & -            & - &-  &-      &-              \\
				
				\hline
				\cite{zouaq2011towards}     & \cmark     & -            & \cmark   & - & -  &-             &  -  & -     & -     & \cmark             &   -  &  -&\cmark   & -            & - &-  &Concept maps      &-              \\
				
				\hline
				\cite{hasan2014generating}   & \cmark     & -            & -   & - & -  &-             &  -  & -     & -     & -             &   -  &  -&-   & -            & - &-  &Sub-graph      &-              \\
				
				\hline
				\cite{graves2008method}    & \cmark     & \cmark            & -   & - & -  &-             &  -  & -     & -     & -             &   -  &  -&-   & -            & - &-  &RDF graph      &-              \\
				
				\bottomrule
			\end{tabular}
			\begin{tablenotes}
				
				\item[1] Degree Centrality.
				\item[2] Closeness Centrality.
				\item[3] Betweenness Centrality.
				\item[4] Bridging Centrality.
				\item[5] Harmonic Centrality.
				\item[6] Radiality.
				\item[7] Ego Centrality.
				\item[8] Relative Cardinality.
				\item[9] Relevance.
				\item[10] Eigenvector Centrality.
				\item[11] Frequency.
				\item[12] Name Simplicity.
				\item[13] Density.
				\item[14] Coverage.
				\item[15] Popularity.
				\item[16] Reference.
				
			\end{tablenotes}
		\end{threeparttable}
	}
	
	
	
	\label{OntoSum}
\end{table*}
\fi

%****************************************************************************************
\subsection{RDF sentence based approach  }
In \cite{zhang2007ontology,zhang2009summarizing}, an RDF sentence is considered as a basic building block in generating ontology summary. The proposed model consists of four main components including \emph{RDF sentence Builder}, \emph{Graph Builder}, \emph{Salience Assessor}, and \emph{Re-ranker}. The key point in this approach is that the user preference will be discussed to determine the weight of links between RDF sentences. In fact,  from \emph{RDF sentence Builder} and \emph{Graph Builder} components the ontology is mapped to a set of RDF sentences and an RDF Sentence Graph is build based on set of RDF sentences and user's preference. The \emph{Salience Assessor} component is responsible to do link analysis on RDF Sentence Graph, generated from the previous component, in order to assess the salience of RDF sentences. This component applies \emph{Degree Centrality, Betweenness Centrality, and Eigenvector Centrality} to assess the RDF sentences and finally, rank them according to their salience. \emph{Re-ranker} component in the last step generate the final summary of the ontology. The coherence of the summary and its coverage on the original ontology are also considered in this section in addition to user-specified salient RDF sentences.
To evaluate the proposed approach the authors used Kendall's tau Statistic \cite{sheskin2003handbook} to measure the agreement between the model's output and human generated results.
%Multi-agent systems \cite{obitko2002ontologies} and data integration \cite{gagnon2007ontology} are two examples of reusing ontological knowledge in order to develop new ontologies.  

%****************************************************************************************
\subsection{Personalized Ontology Summary  }
Queiroz-Sousa et al. \cite{queiroz2013method} defines two steps in ontology summarization including finding key concepts and select them to generate a summary.  For the first step, identifying key concepts,  they introduce \emph{relevance measurement} which is inspired from two main measurements including Degree Centrality and Closeness Centrality (equation \ref{eq:person}).
\begin{equation}
\label{eq:person}
\emph{relevance(C)}=\beta * \emph{DC(C)} + \alpha * \emph{CC(C)}
\end{equation}
Where $\alpha +\beta=1$. In the second step, they develop \emph{Broaden Relevant Paths} (BRP) algorithm in order to find the best path within an ontology that represents a set of interrelated vertices with higher relevance. The BRP algorithm aims to generate three lists including \emph{PathSet, NodeSet, and AdjacentNodes}. The \emph{PathSet} list stores the best paths generated by the algorithm. The quality of each path is defined through two metrics including \emph{Relevance Coverage} and \emph{Relevance Degree}. The \emph{Relevance Coverage} is determined by the proportion of the sum of vertices' relevance within a path by the sum of relevance of the vertices with in the original graph. \emph{Relevance Degree} assesses the relevance average within a path by the higher value of relevance in the graph. The \emph{NodeSet} covers all vertices ordered by their relevance values and the \emph{AdjacentNodes} includes the vertices that have relationships with the vertices of paths contained in the \emph{PathSet}. The \emph{AdjacentNodes} arrange the vertices based on \emph{Relation Relevance} score and the \emph{Relation Relevance} is a function of the number of relationships among a vertex and the paths contained in  \emph{PathSet}, the sum of relevance values of that vertex in a particular path over the number of vertices contained in the \emph{PathSet} list, and finally, the relevance of that vertex. The ultimate summary in this approach containing the most relevant concepts with respect to all relationships between those concepts while considering the parameters set by the user.

%****************************************************************************************
\subsection{Ontology-Based Schemas in PDMS  }
In Pires et al. \cite{pires2010summarizing} model, degree centrality and frequency measurements are two key points to generate a summary for an ontology. They have applied the extended version of degree centrality in which the type of relationships between concepts are considered in addition to number of relations that each concept has. The frequency measure of each concept in this model also determines the importance of each concept and the combination of two measurements is define as \emph{relevance} score of that concept.
\begin{equation}
\label{eq:emc}
\emph{relevance(C)}=\lambda.\emph{DC(C)} + \beta * \emph{Fr(C)}
\end{equation}
Where $\lambda +\beta=1$. The relevance score of each concept needs to be greater than or equal to relevance score threshold to be considered as a good candidate for the final summary. Finding group adjacent relevant concepts and identifying paths between those groups of concepts are two phases after assigning a relevance score to each concept. 


%****************************************************************************************
\subsection{Ontology Summarization: An Analysis and An Evaluation  }
Li et al. \cite{li2010ontology}, highlights the lack of consensus in ontology summarization area and try to come up with a generalized approach for ontology summarization while focusing more on facilitating user understanding of ontology using a few space as possible. They mainly concentrate on \emph{linguistic} and \emph{structural} aspects on ontology as the primary features to be looked in ontology summarization.
In light of \emph{linguistic} aspects, \emph{popularity} and \emph{name simplicity} are two criteria to be discussed and \emph{density} and \emph{reference} are two other criteria that need to be considered with respect to \emph{structural} aspects on ontology. For their evaluation they used Kendall's tau Statistic \cite{sheskin2003handbook} which is often applied to calculate the agreements between two measured quantities. 

%****************************************************************************************
\subsection{Identifying Key Concepts within an Ontology  }
Automatically identifying the key concepts within an ontology applying topological and lexical criteria including \emph{Name Simplicity, Density, Coverage,} and \emph{Popularity}  is the main idea behind \cite{pires2010summarizing} approach. The ultimate goal in Pires et al. \cite{pires2010summarizing} model is to return a subset of concept from an ontology that match as much as possible to those concepts produced by human experts. This model is focusing more on returning key concepts within an ontology without pay that much attention to generating a graph of extracted important concepts.
%****************************************************************************************
% \subsection{Identifying Key Concepts within an Ontology  }
% Automatically identifying the key concepts within an ontology applying topological and lexical criteria including \emph{Name Simplicity, Density, Coverage,} and \emph{Popularity}  is the main idea behind \cite{pires2010summarizing} approach. The ultimate goal in Pires et al. \cite{pires2010summarizing} model is to return a subset of concept from an ontology that match as much as possible to those concepts produced by human experts. This model is focusing more on returning key concepts within an ontology without pay that much attention to generating a graph of extracted important concepts.
%****************************************************************************************
\subsection{Ontology Understanding without Tears  }
Troullinou et al. in \cite{troullinou2017ontology} proposed an advanced version of \emph{RDF Digest: Efficient summarization of RDF/S KBs} \cite{troullinou2015rdf} as a new automatically high quality RDF/S Knowledge Bases summary producer. Finding the most representative concepts within schema graph considering the corresponding instances is the key point in generating the summary for an ontology. In this context, the \emph{structure} of the graph and \emph{semantics} of KB are playing important roles in the final summary. In the proposed approach, the importance of each node (concept) is determined through the \emph{Relative Cardinality}, in the next step the centrality of each node in the KB is estimated by combining the \emph{Relative Cardinality} with the type and number of the \emph{incoming } and \emph{outgoing}edges in the schema. The final step in this approach is generating valid sub-schema graphs that cover more relevant nodes by minimizing their overlaps. Two algorithms that try to optimize the local and global importance of the selected paths are applied in order to generate the final summarized sub-schema graphs.
%****************************************************************************************

% %****************************************************************************************
% \section{The potential role of Topic Modeling in Ontology Summarization }
% Recently, the topic modeling approach has become a popular method for uncovering the hidden themes from data such as text corpora, images, etc. This model has been widely used for various text mining tasks, such as machine translation, word embedding, automatic topic labeling, and many others. In the topic modeling approach, each document is considered as a mixture of topics, where a topic is a probability distribution over words. When the topic proportions of documents are estimated, they can be used as the themes (high-level semantics) of the documents. 

% Ontology Summarization with respect to using topic modeling techniques can be highlighted from various point of views as follows. 
% %****************************************************************************************
% \subsection{Extractive vs Non-Extractive }
% The current ontology summarization models apply extractive method to generate a summary for an ontology. It means that the final summary will contains key concepts of the original ontology. This approach is applicable but there is a chance that the extracted concepts can not represent the underline ontology (gene ontology in biology domain) properly. In this scenario, combining extra knowledge with the extracted concepts from the ontology in order to generate a more representative summary would lead to a better result.  It is the case that by applying topic modeling techniques, we can define a \emph{K} representative topics for an ontology while using the extracted concepts. Applying this model can be consider as a non-extractive technique for ontology summarization. 
% %****************************************************************************************
% \subsection{Unsupervised learning method }
% The available ontology summarization methods are based on some quantitative measures in which the importance of nodes are calculated and the most important ones are selected as a summary. Applying available or extra knowledge through machine learning technique is a potential approach to be considered as a way to generate more reliable summary for an ontology. Topic modeling in this scenario as an unsupervised machine learning technique can be discussed.  

